What can we learn about SARS-CoV-2 prevalence from testing and hospital data?

Measuring the prevalence of active SARS-CoV-2 infections in the general population is difficult because tests are conducted on a small and non-random segment of the population. However, people admitted to the hospital for non-COVID reasons are tested at very high rates, even though they do not appear to be at elevated risk of infection. This sub-population may provide valuable evidence on prevalence in the general population. We estimate upper and lower bounds on the prevalence of the virus in the general population and the population of non-COVID hospital patients under weak assumptions on who gets tested, using Indiana data on hospital inpatient records linked to SARS-CoV-2 virological tests. The non-COVID hospital population is tested fifty times as often as the general population, yielding much tighter bounds on prevalence. We provide and test conditions under which this non-COVID hospitalization bound is valid for the general population. The combination of clinical testing data and hospital records may contain much more information about the state of the epidemic than has been previously appreciated. The bounds we calculate for Indiana could be constructed at relatively low cost in many other states.

==> errorRates.tex <==

PUNCHLINE: Negative predictive value appears very high in our sample, above 99 percent.

A BIT MORE DETAIL. AMONG PEOPLE TESTED EXACTLY TWICE WITHIN A 2-DAY PERIOD, ASSUMING PREVALENCE IS CONSTANT AND THERE ARE NO FALSE POSITIVES, PREVALENCE = 0.12, FALSE NEGATIVE RATE = 0.04, NEGATIVE PREDICTIVE VALUE = 0.995.



Suppose we observe two tests for each person, $d_{1i}$ and$d_{2i}$. Assume status doesn't change between tests, and $C_i$ indicates status. Let $p$ be prevalence=$Pr(C_i=1)$. Let $TPR$ be the true positive rate $Pr(d_{ji}=1|C_{i}=1)$, and $TNR$ the true negative rate, $Pr(d_{ji}=0|C_i=0)$. Note that we implicitly assume the conditional independence of the errors, given type.

There are four possible sequences of outcomes, which we denote $00, 01, 10, 11$. Let $P_{11}$, etc., indicate the probabilities of these outcomes, assuming random testing and retesting. Notice that $P_{01}=P_{10}$ and the probabilities sum to 1, so the only non-redundant probabilities are
\begin{align*}
P_{00} & = (1-p)TNR^2 + p(1-TPR)^2 \\
P_{11} & = (1-p)(1-TNR)^2 + p TPR^2.
\end{align*}
Notice that we have two equations in three unknowns so two tests do not jointly identify error rates and prevalence without further restrictions. (This is an instance of a general result from measurement error theory that three measures are required for identification; see e.g. \cite{HuBook2020}.)  We invoke the assumption that $TNR=1$, i.e. that there are no false positives. \cite{ManskiMolinari2020} make a similar assumption, citing interviews and reports from experts. XXX MAYBE DISCUSS EVIDENCE ON SPECIFICITY XXX.

Under this assumption, we have
\begin{align*}
p  & = \frac{ (P_{00}-P_{11} -2 TNR)^2  }%
    {4 (-P_{00} + TNR + P_{00} TNR - P_{11} TNR - TNR^2)  } \\
TPR & = \frac{2 P_{11}}{1 - P_{00} + P_{11} }
\end{align*}
This shows how to get $p$ and $TPR$ from two tests and $TNR=1$. Our goal is to find the negative predictive value, but we can calculate it given knowledge of $TNR, TPR,$ and $p$.

In general the NPV is $Pr(C_i=0|d_i=0)$. By Bayes rule,
\begin{equation*}
NPV = \frac{Pr(d_i=0|C_i=0)Pr(c_i=0)}{Pr(d_i=0)}
\end{equation*} 
so
\begin{equation*}
NPV = \frac{1-p}{p(1-TPR) + (1-p)}
\end{equation*}

To implement this approach, we take all people who are tested on a given day, not tested the previous day, and then tested again in the next day. There are 16,401 such test pairs. We find $P_{00} = 0.88$ and $P_{11}= 0.11$. Nearly all the mass is on the diagonals; test results switch less than 1\% of the time. This fact, together with the assumed $TNR=1$, implies very low false negative rates. Plugging these values into our formula, we have $p=0.12$ and $TPR=0.96$, which imply $NPV = 0.995$.  Using instead, all people who are retested once within a three day period, we find similar results: $p=0.13, TPR=0.91, NPV=0.986$.

==> tables/bounds_by_date_hosp0.tex <==
3/20 & 6,637,426 &  2,612 &  417 &  0.0001 &  0.1598 &  0.9997 \\ 
4/1 & 6,637,426 &  10,634 &  2,286 &  0.0003 &  0.2150 &  0.9987 \\ 
4/29 & 6,637,426 &  22,776 &  3,923 &  0.0006 &  0.1722 &  0.9972 \\ 
6/7 & 6,637,426 &  37,499 &  1,977 &  0.0003 &  0.0527 &  0.9946 \\ 
6/15 & 6,637,426 &  37,389 &  1,418 &  0.0002 &  0.0379 &  0.9946 \\ 


==> tables/bounds_by_date_hosp1.tex <==
3/20 & 585 &  8 &  1 &  0.0015 &  0.1017 &  0.9870 \\ 
4/1 & 454 &  44 &  5 &  0.0104 &  0.1082 &  0.9143 \\ 
4/29 & 468 &  93 &  6 &  0.0119 &  0.0597 &  0.8126 \\ 
6/7 & 570 &  149 &  2 &  0.0043 &  0.0163 &  0.7438 \\ 
6/15 & 453 &  113 &  2 &  0.0044 &  0.0177 &  0.7553 \\ 


==> tables/bounds_by_dx.tex <==
Blood diseases & 741 &  0.009 &  0.040 &  0.775 &  0.013 &  0.041 &  0.698 &  0.010 &  0.025 &  0.604 \\ 
Circulatory system & 7,743 &  0.008 &  0.045 &  0.837 &  0.012 &  0.037 &  0.687 &  0.009 &  0.025 &  0.644 \\ 
Digestive system & 5,151 &  0.001 &  0.013 &  0.904 &  0.010 &  0.033 &  0.717 &  0.007 &  0.020 &  0.651 \\ 
Endocrine/nutritional/metabolic diseases & 2,798 &  0.021 &  0.123 &  0.849 &  0.046 &  0.135 &  0.704 &  0.024 &  0.072 &  0.685 \\ 
Factors influencing health/contact w/health services & 1,514 &  0.018 &  0.242 &  0.943 &  0.034 &  0.165 &  0.828 &  0.043 &  0.148 &  0.754 \\ 
Genitourinary system & 3,109 &  0.020 &  0.125 &  0.862 &  0.023 &  0.072 &  0.705 &  0.013 &  0.036 &  0.649 \\ 
Infectious diseases & 4,032 &  0.350 &  0.550 &  0.714 &  0.252 &  0.481 &  0.727 &  0.202 &  0.310 &  0.551 \\ 
Injury, poising, other external causes & 3,736 &  0.008 &  0.054 &  0.870 &  0.008 &  0.028 &  0.722 &  0.006 &  0.018 &  0.644 \\ 
Mental/behavioral/neurodevelopment & 2,315 &  0.003 &  0.048 &  0.943 &  0.001 &  0.007 &  0.810 &  0.003 &  0.013 &  0.736 \\ 
Musculoskeletal system and connective tissue & 1,599 &  0.005 &  0.095 &  0.951 &  0.013 &  0.051 &  0.751 &  0.004 &  0.012 &  0.713 \\ 
Neoplasms & 1,822 &  0.003 &  0.043 &  0.926 &  0.000 &  0.000 &  0.743 &  0.002 &  0.006 &  0.736 \\ 
Nervous system & 1,526 &  0.007 &  0.041 &  0.830 &  0.010 &  0.039 &  0.754 &  0.015 &  0.049 &  0.716 \\ 
Perinatal conditions & 5,752 &  0.000 &  0.000 &  0.996 &  0.000 &  0.000 &  0.992 &  0.000 &  0.059 &  0.992 \\ 
Pregnancy, childbirth, and the peurperium & 6,684 &  0.002 &  0.104 &  0.981 &  0.003 &  0.025 &  0.893 &  0.006 &  0.031 &  0.805 \\ 
Respiratory system & 4,673 &  0.108 &  0.210 &  0.591 &  0.075 &  0.114 &  0.413 &  0.057 &  0.080 &  0.344 \\ 
Skin and subcutaneous tissue & 968 &  0.000 &  0.000 &  0.914 &  0.003 &  0.013 &  0.735 &  0.012 &  0.041 &  0.716 \\ 
Symptoms etc. not elsewhere classified & 5,450 &  0.080 &  0.295 &  0.808 &  0.062 &  0.138 &  0.617 &  0.040 &  0.089 &  0.591 \\ 
Uncategorized/invalid primary DX & 347 &  0.008 &  0.111 &  0.936 &  0.010 &  0.067 &  0.867 &  0.017 &  0.074 &  0.786 \\ 


==> tables/bounds_by_group.tex <==
3/13/2020 &  0.0001 &  0.113 &  0.0030 &  0.090 &  0.0022 &  0.073 &  0.0717 &  0.244 \\ 
3/20/2020 &  0.0003 &  0.181 &  0.0163 &  0.159 &  0.0148 &  0.174 &  0.2868 &  0.395 \\ 
3/27/2020 &  0.0006 &  0.196 &  0.0330 &  0.209 &  0.0210 &  0.147 &  0.4308 &  0.517 \\ 
4/03/2020 &  0.0006 &  0.177 &  0.0279 &  0.161 &  0.0258 &  0.163 &  0.3529 &  0.444 \\ 
4/10/2020 &  0.0006 &  0.168 &  0.0254 &  0.134 &  0.0184 &  0.106 &  0.3105 &  0.402 \\ 
4/17/2020 &  0.0008 &  0.187 &  0.0166 &  0.084 &  0.0126 &  0.058 &  0.2636 &  0.366 \\ 
4/24/2020 &  0.0008 &  0.146 &  0.0217 &  0.110 &  0.0153 &  0.086 &  0.2694 &  0.419 \\ 
5/01/2020 &  0.0009 &  0.125 &  0.0165 &  0.058 &  0.0187 &  0.057 &  0.2467 &  0.326 \\ 
5/08/2020 &  0.0008 &  0.097 &  0.0120 &  0.039 &  0.0154 &  0.047 &  0.1901 &  0.255 \\ 
5/15/2020 &  0.0008 &  0.094 &  0.0145 &  0.045 &  0.0190 &  0.057 &  0.1826 &  0.240 \\ 
5/22/2020 &  0.0006 &  0.084 &  0.0143 &  0.047 &  0.0164 &  0.053 &  0.1913 &  0.261 \\ 
5/29/2020 &  0.0006 &  0.069 &  0.0090 &  0.028 &  0.0089 &  0.027 &  0.1415 &  0.192 \\ 
6/05/2020 &  0.0006 &  0.056 &  0.0085 &  0.026 &  0.0087 &  0.027 &  0.1608 &  0.216 \\ 
6/12/2020 &  0.0005 &  0.041 &  0.0057 &  0.018 &  0.0070 &  0.023 &  0.1312 &  0.187 \\ 
6/19/2020 &  0.0006 &  0.049 &  0.0057 &  0.018 &  0.0048 &  0.015 &  0.1118 &  0.161 \\ 
6/26/2020 &  0.0006 &  0.058 &  0.0062 &  0.020 &  0.0102 &  0.031 &  0.1152 &  0.163 \\ 
7/03/2020 &  0.0007 &  0.067 &  0.0047 &  0.015 &  0.0084 &  0.026 &  0.1291 &  0.183 \\ 
7/10/2020 &  0.0009 &  0.067 &  0.0066 &  0.020 &  0.0082 &  0.024 &  0.1416 &  0.205 \\ 
7/17/2020 &  0.0010 &  0.069 &  0.0054 &  0.017 &  0.0066 &  0.020 &  0.1471 &  0.208 \\ 
7/24/2020 &  0.0010 &  0.072 &  0.0083 &  0.027 &  0.0119 &  0.039 &  0.1626 &  0.228 \\ 
7/31/2020 &  0.0011 &  0.071 &  0.0088 &  0.028 &  0.0110 &  0.035 &  0.1692 &  0.251 \\ 
8/07/2020 &  0.0010 &  0.067 &  0.0070 &  0.023 &  0.0097 &  0.030 &  0.1606 &  0.242 \\ 
8/14/2020 &  0.0010 &  0.061 &  0.0068 &  0.023 &  0.0137 &  0.047 &  0.1454 &  0.224 \\ 
8/21/2020 &  0.0010 &  0.064 &  0.0063 &  0.022 &  0.0090 &  0.031 &  0.1490 &  0.230 \\ 
8/28/2020 &  0.0010 &  0.066 &  0.0061 &  0.022 &  0.0058 &  0.021 &  0.1238 &  0.201 \\ 
9/04/2020 &  0.0009 &  0.060 &  0.0068 &  0.024 &  0.0073 &  0.025 &  0.1304 &  0.205 \\ 
9/11/2020 &  0.0009 &  0.055 &  0.0056 &  0.019 &  0.0093 &  0.030 &  0.1337 &  0.205 \\ 
9/18/2020 &  0.0009 &  0.059 &  0.0064 &  0.021 &  0.0093 &  0.032 &  0.1321 &  0.208 \\ 
9/25/2020 &  0.0012 &  0.072 &  0.0073 &  0.024 &  0.0095 &  0.031 &  0.1340 &  0.215 \\ 
10/02/2020 &  0.0015 &  0.082 &  0.0080 &  0.026 &  0.0099 &  0.032 &  0.1840 &  0.280 \\ 
10/09/2020 &  0.0017 &  0.102 &  0.0103 &  0.034 &  0.0153 &  0.051 &  0.2342 &  0.357 \\ 
10/16/2020 &  0.0024 &  0.111 &  0.0126 &  0.038 &  0.0150 &  0.046 &  0.2502 &  0.392 \\ 
10/23/2020 &  0.0031 &  0.134 &  0.0162 &  0.047 &  0.0236 &  0.069 &  0.2876 &  0.435 \\ 
10/30/2020 &  0.0042 &  0.163 &  0.0145 &  0.044 &  0.0216 &  0.067 &  0.3130 &  0.513 \\ 
11/06/2020 &  0.0055 &  0.191 &  0.0259 &  0.071 &  0.0357 &  0.105 &  0.3728 &  0.582 \\ 
11/13/2020 &  0.0059 &  0.184 &  0.0281 &  0.065 &  0.0530 &  0.114 &  0.4215 &  0.626 \\ 
11/20/2020 &  0.0053 &  0.198 &  0.0391 &  0.093 &  0.0532 &  0.116 &  0.3983 &  0.602 \\ 
11/27/2020 &  0.0066 &  0.227 &  0.0381 &  0.084 &  0.0699 &  0.142 &  0.4170 &  0.621 \\ 
12/04/2020 &  0.0047 &  0.214 &  0.0310 &  0.069 &  0.0531 &  0.108 &  0.4261 &  0.637 \\ 
12/11/2020 &  0.0010 &  0.196 &  0.0206 &  0.051 &  0.0397 &  0.085 &  0.3570 &  0.599 \\ 


==> tables/bounds_by_group_wtd.tex <==
3/13/2020 &  0.0001 &  0.097 &  0.0019 &  0.043 &  0.0017 &  0.044 &  0.0609 &  0.180 \\ 
3/20/2020 &  0.0003 &  0.154 &  0.0139 &  0.112 &  0.0107 &  0.110 &  0.2300 &  0.309 \\ 
3/27/2020 &  0.0006 &  0.166 &  0.0286 &  0.159 &  0.0148 &  0.113 &  0.3281 &  0.392 \\ 
4/03/2020 &  0.0006 &  0.154 &  0.0238 &  0.131 &  0.0135 &  0.083 &  0.2723 &  0.339 \\ 
4/10/2020 &  0.0006 &  0.149 &  0.0236 &  0.138 &  0.0132 &  0.169 &  0.2599 &  0.335 \\ 
4/17/2020 &  0.0008 &  0.169 &  0.0115 &  0.051 &  0.0054 &  0.026 &  0.1980 &  0.268 \\ 
4/24/2020 &  0.0008 &  0.137 &  0.0182 &  0.086 &  0.0108 &  0.057 &  0.2638 &  0.404 \\ 
5/01/2020 &  0.0009 &  0.122 &  0.0153 &  0.049 &  0.0192 &  0.064 &  0.2499 &  0.322 \\ 
5/08/2020 &  0.0008 &  0.096 &  0.0119 &  0.035 &  0.0215 &  0.093 &  0.1744 &  0.231 \\ 
5/15/2020 &  0.0008 &  0.099 &  0.0120 &  0.035 &  0.0121 &  0.043 &  0.1675 &  0.216 \\ 
5/22/2020 &  0.0006 &  0.087 &  0.0158 &  0.051 &  0.0110 &  0.040 &  0.1607 &  0.217 \\ 
5/29/2020 &  0.0006 &  0.073 &  0.0083 &  0.025 &  0.0070 &  0.022 &  0.1474 &  0.206 \\ 
6/05/2020 &  0.0006 &  0.059 &  0.0073 &  0.022 &  0.0064 &  0.021 &  0.1541 &  0.203 \\ 
6/12/2020 &  0.0005 &  0.045 &  0.0067 &  0.022 &  0.0053 &  0.018 &  0.1192 &  0.166 \\ 
6/19/2020 &  0.0006 &  0.051 &  0.0047 &  0.014 &  0.0046 &  0.016 &  0.1129 &  0.153 \\ 
6/26/2020 &  0.0006 &  0.060 &  0.0070 &  0.022 &  0.0071 &  0.021 &  0.1210 &  0.168 \\ 
7/03/2020 &  0.0007 &  0.069 &  0.0049 &  0.015 &  0.0088 &  0.033 &  0.1347 &  0.188 \\ 
7/10/2020 &  0.0009 &  0.067 &  0.0086 &  0.026 &  0.0067 &  0.020 &  0.1292 &  0.188 \\ 
7/17/2020 &  0.0010 &  0.069 &  0.0041 &  0.011 &  0.0042 &  0.012 &  0.1269 &  0.179 \\ 
7/24/2020 &  0.0010 &  0.072 &  0.0064 &  0.019 &  0.0065 &  0.021 &  0.1522 &  0.204 \\ 
7/31/2020 &  0.0011 &  0.072 &  0.0104 &  0.034 &  0.0110 &  0.052 &  0.1270 &  0.183 \\ 
8/07/2020 &  0.0010 &  0.067 &  0.0087 &  0.032 &  0.0065 &  0.020 &  0.1127 &  0.170 \\ 
8/14/2020 &  0.0010 &  0.059 &  0.0070 &  0.022 &  0.0173 &  0.066 &  0.1283 &  0.184 \\ 
8/21/2020 &  0.0010 &  0.060 &  0.0066 &  0.022 &  0.0098 &  0.041 &  0.1278 &  0.191 \\ 
8/28/2020 &  0.0010 &  0.062 &  0.0052 &  0.016 &  0.0035 &  0.012 &  0.1006 &  0.154 \\ 
9/04/2020 &  0.0009 &  0.057 &  0.0049 &  0.016 &  0.0042 &  0.015 &  0.1198 &  0.182 \\ 
9/11/2020 &  0.0009 &  0.053 &  0.0053 &  0.016 &  0.0043 &  0.014 &  0.0830 &  0.127 \\ 
9/18/2020 &  0.0009 &  0.058 &  0.0051 &  0.016 &  0.0064 &  0.022 &  0.0879 &  0.141 \\ 
9/25/2020 &  0.0012 &  0.070 &  0.0064 &  0.019 &  0.0061 &  0.018 &  0.0993 &  0.154 \\ 
10/02/2020 &  0.0014 &  0.081 &  0.0058 &  0.018 &  0.0065 &  0.024 &  0.1364 &  0.210 \\ 
10/09/2020 &  0.0017 &  0.101 &  0.0086 &  0.027 &  0.0072 &  0.021 &  0.1975 &  0.297 \\ 
10/16/2020 &  0.0024 &  0.110 &  0.0103 &  0.029 &  0.0073 &  0.022 &  0.1747 &  0.277 \\ 
10/23/2020 &  0.0031 &  0.132 &  0.0115 &  0.030 &  0.0154 &  0.047 &  0.2028 &  0.305 \\ 
10/30/2020 &  0.0042 &  0.162 &  0.0136 &  0.038 &  0.0190 &  0.057 &  0.2422 &  0.406 \\ 
11/06/2020 &  0.0055 &  0.189 &  0.0213 &  0.056 &  0.0230 &  0.069 &  0.3045 &  0.487 \\ 
11/13/2020 &  0.0059 &  0.181 &  0.0264 &  0.060 &  0.0450 &  0.115 &  0.3206 &  0.486 \\ 
11/20/2020 &  0.0052 &  0.196 &  0.0352 &  0.080 &  0.0519 &  0.160 &  0.3169 &  0.490 \\ 
11/27/2020 &  0.0066 &  0.225 &  0.0306 &  0.062 &  0.0457 &  0.100 &  0.3500 &  0.536 \\ 
12/04/2020 &  0.0047 &  0.213 &  0.0243 &  0.048 &  0.0299 &  0.060 &  0.3432 &  0.502 \\ 
12/11/2020 &  0.0010 &  0.195 &  0.0277 &  0.056 &  0.0480 &  0.086 &  0.2589 &  0.408 \\ 


==> tables/bounds_no_icli.tex <==
March & 16,813 &  0.087 &  0.015 &  0.173\\ 
April & 24,980 &  0.187 &  0.023 &  0.124\\ 
May & 32,018 &  0.305 &  0.014 &  0.046\\ 
June & 35,793 &  0.321 &  0.007 &  0.021\\ 
July & 38,190 &  0.317 &  0.006 &  0.020\\ 
August & 37,705 &  0.300 &  0.007 &  0.024\\ 
September & 37,548 &  0.298 &  0.006 &  0.021\\ 
October & 36,717 &  0.321 &  0.012 &  0.036\\ 
November & 33,342 &  0.397 &  0.029 &  0.073\\ 
December & 12,415 &  0.444 &  0.030 &  0.067\\ 


==> tables/cfr_estimates.tex <==
March-April & .0068 &   .0875 &   .9289 &   14.1045 &   .0002 &   .0016 &   .0207 \\  
April-May & .0088 &   .0416 &   .7969 &   14.6866 &   .0002 &   .0035 &   .0167 \\  
May-June & .0059 &   .0234 &   .7524 &   7.0299 &   .0001 &   .0030 &   .0118 \\  


==> tables/county_test_rates.tex <==
    \underline{Population} \\ Average person &        .267   \\ \\ \underline{Hospitalizations} \\  
                   Non-ICLI hospitalization  &        .266                                      \\  
                                             &    [20.8]                                      \\  
                Clear cause hospitalization  &        .265                                      \\  
                                             &    [16.9]                                      \\  
                       ICLI hospitalization  &        .267                                      \\  
                                             &     [2.5]                                      \\  



==> tables/dx_counts.tex <==
DXs & 2,677,804\\
Encounters & 446,839\\
Patients & 325,410\\


==> tables/hospital_variability.tex <==
SD & 0.14 &  0.16 &  0.16 \\ 
Interquartile range & 0.17 &  0.22 &  0.25 \\ 
\\   
Regression statistics \\   
Regression $R^2 $ & 0.06 &  0.18 &  0.19 \\ 
\# of hospitals & 70 &  70 &  70 \\ 
\# Hospitalizations & 384,219 &  384,219 &  384,219 \\ 


==> tables/predictivity_out_of_sample_mse.tex <==
New positive tests & 11.2 &  15.8 &  16.9 &  19.9 \\ 
Hospital positivity & 19.6 &  16.3 &  11.4 &  10.7 \\ 
Deaths & 0.0 &  12.6 &  15.7 &  21.3 \\ 
Tests + Hospital & 11.1 &  12.1 &  8.5 &  15.3 \\ 
Deaths + positives + hospital & 0.0 &  8.3 &  6.0 &  12.5 \\ 


==> tables/prior_rates.tex <==
3/13/2020 &  0.000 &  0.000  (0.000, 0.000) & 0.000  (0.000, 0.000) & 0.000  (0.000, 0.000) \\
3/20/2020 &  0.000 &  0.001  (0.000, 0.003) & 0.000  (0.000, 0.000) & 0.001  (0.000, 0.005) \\
3/27/2020 &  0.002 &  0.003  (0.000, 0.007) & 0.003  (0.000, 0.010) & 0.007  (0.000, 0.026) \\
4/03/2020 &  0.004 &  0.002  (0.000, 0.005) & 0.002  (0.000, 0.009) & 0.026  (0.000, 0.066) \\
4/10/2020 &  0.005 &  0.008  (0.000, 0.019) & 0.002  (0.000, 0.008) & 0.008  (0.000, 0.021) \\
4/17/2020 &  0.006 &  0.010  (0.000, 0.025) & 0.017  (0.000, 0.051) & 0.021  (0.000, 0.042) \\
4/24/2020 &  0.007 &  0.007  (0.001, 0.013) & 0.005  (0.000, 0.015) & 0.024  (0.001, 0.047) \\
5/01/2020 &  0.009 &  0.014  (0.001, 0.027) & 0.030  (0.000, 0.082) & 0.037  (0.000, 0.096) \\
5/08/2020 &  0.011 &  0.012  (0.003, 0.022) & 0.011  (0.000, 0.025) & 0.054  (0.002, 0.106) \\
5/15/2020 &  0.013 &  0.016  (0.006, 0.025) & 0.014  (0.000, 0.039) & 0.054  (0.000, 0.132) \\
5/22/2020 &  0.014 &  0.015  (0.005, 0.024) & 0.008  (0.000, 0.020) & 0.030  (0.000, 0.068) \\
5/29/2020 &  0.014 &  0.014  (0.006, 0.021) & 0.011  (0.000, 0.025) & 0.038  (0.004, 0.071) \\
6/05/2020 &  0.014 &  0.014  (0.004, 0.023) & 0.010  (0.000, 0.024) & 0.030  (0.000, 0.086) \\
6/12/2020 &  0.016 &  0.019  (0.008, 0.030) & 0.012  (0.000, 0.027) & 0.044  (0.000, 0.094) \\
6/19/2020 &  0.019 &  0.018  (0.006, 0.030) & 0.012  (0.000, 0.026) & 0.031  (0.000, 0.064) \\
6/26/2020 &  0.021 &  0.019  (0.009, 0.029) & 0.013  (0.000, 0.028) & 0.031  (0.000, 0.061) \\
7/03/2020 &  0.021 &  0.020  (0.006, 0.035) & 0.012  (0.000, 0.027) & 0.024  (0.000, 0.053) \\
7/10/2020 &  0.018 &  0.015  (0.005, 0.026) & 0.019  (0.000, 0.047) & 0.050  (0.000, 0.102) \\
7/17/2020 &  0.020 &  0.020  (0.006, 0.034) & 0.022  (0.000, 0.060) & 0.022  (0.000, 0.049) \\
7/24/2020 &  0.024 &  0.021  (0.007, 0.034) & 0.014  (0.000, 0.044) & 0.023  (0.000, 0.049) \\
7/31/2020 &  0.026 &  0.025  (0.010, 0.039) & 0.024  (0.000, 0.054) & 0.049  (0.000, 0.111) \\
8/07/2020 &  0.026 &  0.021  (0.008, 0.035) & 0.007  (0.000, 0.018) & 0.064  (0.000, 0.143) \\
8/14/2020 &  0.026 &  0.021  (0.010, 0.032) & 0.016  (0.000, 0.032) & 0.076  (0.000, 0.168) \\
8/21/2020 &  0.028 &  0.020  (0.008, 0.032) & 0.017  (0.000, 0.040) & 0.062  (0.007, 0.117) \\
8/28/2020 &  0.029 &  0.022  (0.009, 0.035) & 0.019  (0.000, 0.046) & 0.054  (0.000, 0.125) \\
9/04/2020 &  0.028 &  0.019  (0.005, 0.032) & 0.013  (0.000, 0.030) & 0.030  (0.000, 0.076) \\
9/11/2020 &  0.026 &  0.017  (0.008, 0.027) & 0.019  (0.000, 0.046) & 0.047  (0.000, 0.102) \\
9/18/2020 &  0.026 &  0.024  (0.009, 0.038) & 0.007  (0.000, 0.019) & 0.046  (0.000, 0.104) \\
9/25/2020 &  0.026 &  0.022  (0.008, 0.036) & 0.031  (0.000, 0.070) & 0.039  (0.000, 0.082) \\
10/02/2020 &  0.026 &  0.019  (0.007, 0.031) & 0.021  (0.000, 0.055) & 0.031  (0.000, 0.069) \\
10/09/2020 &  0.028 &  0.020  (0.010, 0.031) & 0.023  (0.000, 0.055) & 0.047  (0.011, 0.082) \\
10/16/2020 &  0.029 &  0.020  (0.007, 0.034) & 0.022  (0.000, 0.054) & 0.066  (0.012, 0.120) \\
10/23/2020 &  0.031 &  0.018  (0.007, 0.028) & 0.026  (0.000, 0.060) & 0.065  (0.004, 0.126) \\
10/30/2020 &  0.036 &  0.028  (0.014, 0.042) & 0.030  (0.000, 0.069) & 0.065  (0.012, 0.118) \\
11/06/2020 &  0.040 &  0.027  (0.012, 0.041) & 0.020  (0.000, 0.049) & 0.080  (0.018, 0.142) \\
11/13/2020 &  0.044 &  0.033  (0.016, 0.051) & 0.048  (0.000, 0.108) & 0.075  (0.038, 0.112) \\
11/20/2020 &  0.050 &  0.037  (0.017, 0.057) & 0.024  (0.001, 0.047) & 0.065  (0.025, 0.105) \\
11/27/2020 &  0.054 &  0.042  (0.021, 0.064) & 0.052  (0.000, 0.111) & 0.080  (0.035, 0.124) \\
12/04/2020 &  0.047 &  0.037  (0.017, 0.056) & 0.033  (0.000, 0.077) & 0.073  (0.027, 0.120) \\
12/11/2020 &  0.044 &  0.038  (0.002, 0.074) & 0.033  (0.000, 0.135) & 0.066  (0.012, 0.120) \\

